Nested Sequents for Provability Logic GLP

We present a proof system for the provability logic GLP in the formalism of nested sequents and prove the cut elimination theorem for it. As an application, we obtain the reduction of GLP to its important fragment called J syntactically.

==> README <==
=== MinionPro Source Distribution ===

    http://developer.berlios.de/projects/minionpro

    Achim Blumensath
    Andreas B\"uhmann
    Michael Zedler

These files are public domain.

Requirements
============

o LCDF Typetools, version 2.62 or better (http://www.lcdf.org/type/)
o fontinst v1.925 or better

Building
========

1) Unpack the archive:

  $ tar -xzvf MinionPro-source.tgz

2) Copy your OpenType font files into the otf directory.

  $ cp /some/path/*.otf otf

3) Run ./scripts/makeall

  $ ./scripts/makeall

makeall has some options to specify which metrics to create:

  --verbose            show warning messages from otftotfm
  --quiet              omit these messages (default)
  --smallcaps          create small caps metrics (default)
  --nosmallcaps        turn --smallcaps off
  --swash              create swash metrics (default)
  --noswash            turn --swash off
  --greek              create greek metrics (default)
  --nogreek            turn --greek off
  --cyrillic           create cyrillic metrics (default)
  --nocyrillic         turn --cyrillic off
  --vietnamese         create vietnamese metrics (default)
  --novietnamese       turn --vietnamese off
  --expanded           create expanded metrics for pdftex
  --noexpanded         turn --expanded off (default)
  --kern               add some missing kerning pairs (default)
  --nokern             use the original Adobe kerning
  --wide-spacing       increase the sidebearings of quote glyphs
  --narrow-spacing     turn --wide-spacing off (default)
  --pack=<glyph-list>  create base fonts to reduce the size of the map file

Installing
==========

1) Run ./scripts/install. You can specify the directory where the files
should be put. The default is $TEXMFLOCAL.

  $ ./scripts/install /usr/local/teTeX/share/texmf-local

2) Add MinionPro.map to your updmap.cfg and run updmap.

3) If you get errors about insufficient memory you might need to
increase the values of font_mem_size and font_max in your TeX
configuration. For most distributions, these can be changed in the file
texmf/web2c/texmf.cnf. For MiKTeX the file is called miktex.ini.

4) Happy TeXing!



==> bussproofs/README <==
bussproofs, version 1.1.

Proof trees in the style of the sequent calculus and other proof systems.

The package allows the construction of proof trees in the style of
the sequent calculus and many other proof systems. One novel
feature of the macros is they support the horizontal alignment
according to some centre point specified with the command \fCenter.
This is the style often used in sequent calculus proofs.

The package works in a Plain TeX document, as well as in LaTeX; an
exposition of the commands available is given in the package file
itself. Documentation is also given in a separate LaTeX/FILE,
BussGuide2.tex/BussGuide2.pdf.

Distribution under the LaTeX Project Public License

The CTAN distribution includes:

bussproofs.sty - version 1.1 of the style files.

BussGuide2.pdf - The documentation by Peter Smith.
BussGuide2.tex - LaTeX source for the documentation.

testbp2.tex - A file used for testing, with examples of usage.
testbp2.pdf - The output of the testbp2.tex

README.txt - This file.

Maintained by Sam Buss
sbuss@math.ucsd.edu


==> fontinst/fontinst-macros.tex <==
\input fontinst.sty

\fontinstcc
\def\metrics_given_encoding#1#2{
   \x_cs\edef{s-afm-name}{#1-#2}
   \if_file_exists{#1.pl}\then
      \generalpltomtx{#1}{#1-#2}{pl}{#2}
   \else
      \if_file_exists{#1.vpl}\then
         \generalpltomtx{#1}{#1-#2}{vpl}{#2}
      \else
         \unsetstr{afm-name}
   \fi\fi
}
\normalcc

% based on mathpazo's haxzplmr.mtx

% \shiftglyph takes five parameters:
%   #1 the name of the glyph
%   #2 the amount of extra space at the left
%   #3 the amount of extra space at the right
%   #4 the amount of extra space for subscripts
%   #5 the amount of extra height
\setcommand\shiftglyph#1#2#3#4#5{
   \resetglyph{#1}
      \movert{#2}
      \glyph{#1}{1000}
      \movert{#4}
      \resetitalic{\add{\italic{#1}}{\sub{#3}{#4}}}
      \resetheight{\add{\height{#1}}{#5}}
   \endresetglyph
}

% \adjustmetrics takes five parameters:
%   #1 the name of the glyph
%   #2 the amount of extra space at the left
%   #3 the amount of extra space at the right
%   #4 the amount of extra space for subscripts
%   #5 the amount by which to shift accents rightwards
%   #6 the amount of extra height
%
\setcommand\adjustmetrics#1#2#3#4#5#6{
   \shiftglyph{#1}{#2}{#3}{#4}{#6}
   \resetkern{#1}{skew}{#5}
}


==> fontinst/make-MnSymbolFI-noopt-sb.tex <==
\input fontinst-macros.tex

\def\installsemiboldnonopt#1#2{%
  \installfont{#1}{%
     MnSymbolF-Bold10                  encoding mn-symbol-f-partialints,%
     #2                                encoding mn-symbol-f,%
     MinionPro-SemiboldIt-integral     encoding mn-tint scaled 1140,%
     MinionPro-SemiboldIt-integral-cn2 encoding mn-dint scaled 1140,%
     mn-intop-semibold-text,%
     mn-intop-semibold-disp-noopt%
  }{mn-symbol-fi}{}{}{}{}{}%
}

\installfonts

  \installsemiboldnonopt{MnSymbolFI-Semibold-NoOpticals5}{MnSymbolF-Bold5}%
  \installsemiboldnonopt{MnSymbolFI-Semibold-NoOpticals6}{MnSymbolF-Bold6}%
  \installsemiboldnonopt{MnSymbolFI-Semibold-NoOpticals7}{MnSymbolF-Bold7}%
  \installsemiboldnonopt{MnSymbolFI-Semibold-NoOpticals8}{MnSymbolF-Bold8}%
  \installsemiboldnonopt{MnSymbolFI-Semibold-NoOpticals9}{MnSymbolF-Bold9}%
  \installsemiboldnonopt{MnSymbolFI-Semibold-NoOpticals10}{MnSymbolF-Bold10}%
  \installsemiboldnonopt{MnSymbolFI-Semibold-NoOpticals12}{MnSymbolF-Bold12}%

\endinstallfonts

\bye


==> fontinst/make-MnSymbolFI-noopt.tex <==
\input fontinst-macros.tex

\def\installnonopt#1#2{%
  \installfont{#1}{%
     MnSymbolF10                   encoding mn-symbol-f-partialints,%
     #2                            encoding mn-symbol-f,%
     MinionPro-It-integral         encoding mn-tint scaled 1100,%
     MinionPro-It-integral-cn2     encoding mn-dint scaled 1100,%
     mn-intop-text,%
     mn-intop-disp-noopt%
  }{mn-symbol-fi}{}{}{}{}{}%
}

\def\installboldnonopt#1#2{%
  \installfont{#1}{%
     MnSymbolF-Bold10                  encoding mn-symbol-f-partialints,%
     #2                                encoding mn-symbol-f,%
     MinionPro-BoldIt-integral         encoding mn-tint scaled 1140,%
     MinionPro-BoldIt-integral-cn2     encoding mn-dint scaled 1140,%
     mn-intop-bold-text,%
     mn-intop-bold-disp-noopt%
  }{mn-symbol-fi}{}{}{}{}{}%
}


\installfonts

  \installnonopt{MnSymbolFI-NoOpticals5}{MnSymbolF5}%
  \installnonopt{MnSymbolFI-NoOpticals6}{MnSymbolF6}%
  \installnonopt{MnSymbolFI-NoOpticals7}{MnSymbolF7}%
  \installnonopt{MnSymbolFI-NoOpticals8}{MnSymbolF8}%
  \installnonopt{MnSymbolFI-NoOpticals9}{MnSymbolF9}%
  \installnonopt{MnSymbolFI-NoOpticals10}{MnSymbolF10}%
  \installnonopt{MnSymbolFI-NoOpticals12}{MnSymbolF12}%
  \installboldnonopt{MnSymbolFI-Bold-NoOpticals5}{MnSymbolF-Bold5}%
  \installboldnonopt{MnSymbolFI-Bold-NoOpticals6}{MnSymbolF-Bold6}%
  \installboldnonopt{MnSymbolFI-Bold-NoOpticals7}{MnSymbolF-Bold7}%
  \installboldnonopt{MnSymbolFI-Bold-NoOpticals8}{MnSymbolF-Bold8}%
  \installboldnonopt{MnSymbolFI-Bold-NoOpticals9}{MnSymbolF-Bold9}%
  \installboldnonopt{MnSymbolFI-Bold-NoOpticals10}{MnSymbolF-Bold10}%
  \installboldnonopt{MnSymbolFI-Bold-NoOpticals12}{MnSymbolF-Bold12}%

\endinstallfonts

\bye


==> fontinst/make-MnSymbolFI.tex <==
\input fontinst-macros.tex

\def\installopt#1#2{%
  \installfont{#1}{%
     MnSymbolF10                       encoding mn-symbol-f-partialints,%
     #2                                encoding mn-symbol-f,%
     MinionPro-It-integral             encoding mn-tint scaled 1100,%
     MinionPro-ItDisp-integral-cn1     encoding mn-dint scaled 1100,%
     mn-intop-text,%
     mn-intop-disp%
  }{mn-symbol-fi}{}{}{}{}{}%
}

\def\installsemiboldopt#1#2{%
  \installfont{#1}{%
     MnSymbolF-Bold10                      encoding mn-symbol-f-partialints,%
     #2                                    encoding mn-symbol-f,%
     MinionPro-SemiboldIt-integral         encoding mn-tint scaled 1140,%
     MinionPro-SemiboldItDisp-integral-cn1 encoding mn-dint scaled 1140,%
     mn-intop-semibold-text,%
     mn-intop-semibold-disp%
  }{mn-symbol-fi}{}{}{}{}{}%
}


\installfonts

  \installopt{MnSymbolFI5}{MnSymbolF5}%
  \installopt{MnSymbolFI6}{MnSymbolF6}%
  \installopt{MnSymbolFI7}{MnSymbolF7}%
  \installopt{MnSymbolFI8}{MnSymbolF8}%
  \installopt{MnSymbolFI9}{MnSymbolF9}%
  \installopt{MnSymbolFI10}{MnSymbolF10}%
  \installopt{MnSymbolFI12}{MnSymbolF12}%
  \installsemiboldopt{MnSymbolFI-Semibold5}{MnSymbolF-Bold5}%
  \installsemiboldopt{MnSymbolFI-Semibold6}{MnSymbolF-Bold6}%
  \installsemiboldopt{MnSymbolFI-Semibold7}{MnSymbolF-Bold7}%
  \installsemiboldopt{MnSymbolFI-Semibold8}{MnSymbolF-Bold8}%
  \installsemiboldopt{MnSymbolFI-Semibold9}{MnSymbolF-Bold9}%
  \installsemiboldopt{MnSymbolFI-Semibold10}{MnSymbolF-Bold10}%
  \installsemiboldopt{MnSymbolFI-Semibold12}{MnSymbolF-Bold12}%
%  \installboldopt{MnSymbolFI-Bold5}{MnSymbolF-Bold5}%
%  \installboldopt{MnSymbolFI-Bold6}{MnSymbolF-Bold6}%
%  \installboldopt{MnSymbolFI-Bold7}{MnSymbolF-Bold7}%
%  \installboldopt{MnSymbolFI-Bold8}{MnSymbolF-Bold8}%
%  \installboldopt{MnSymbolFI-Bold9}{MnSymbolF-Bold9}%
%  \installboldopt{MnSymbolFI-Bold10}{MnSymbolF-Bold10}%
%  \installboldopt{MnSymbolFI-Bold12}{MnSymbolF-Bold12}%

\endinstallfonts

\bye


==> fontinst/make-oml-fullfamily-opticals.tex <==
\input fontinst-macros.tex

\def\installopt#1#2#3#4{%
  \installfont{MinionPro-Medium#3#1-#4oml}{%
     MnSymbolA#2                       encoding mn-symbol-a,%
     MnSymbolC#2                       encoding mn-symbol-c,%
     MnSymbolD#2                       encoding mn-symbol-d,%
     MnSymbolE#2                       encoding mn-symbol-e,%
     MinionPro-Medium#1-tosf-#4oml     encoding mn-oml-up,%
     MinionPro-MediumIt#1-tosf-#4oml   encoding mn-oml-it,%
     adjust-oml,%
     arrowhooks,%
     tie%
  }{mn-oml-#3}{}{}{}{}{}%
}

\installfonts
  \installopt{Capt}{7}{Mixed}{l1-}
  \installopt{Capt}{7}{Mixed}{}
  \installopt{Subh}{12}{Mixed}{}
  \installopt{Disp}{12}{Mixed}{}
  \installopt{Capt}{7}{French}{l1-}
  \installopt{Capt}{7}{French}{}
  \installopt{Subh}{12}{French}{}
  \installopt{Disp}{12}{French}{}
\endinstallfonts

\bye


==> fontinst/make-oml-fullfamily.tex <==
\input fontinst-macros.tex

\def\installopt#1#2#3{%
  \installfont{MinionPro-Medium#2-#3oml}{%
     MnSymbolA#1                       encoding mn-symbol-a,%
     MnSymbolC#1                       encoding mn-symbol-c,%
     MnSymbolD#1                       encoding mn-symbol-d,%
     MnSymbolE#1                       encoding mn-symbol-e,%
     MinionPro-Medium-tosf-#3oml       encoding mn-oml-up,%
     MinionPro-MediumIt-tosf-#3oml     encoding mn-oml-it,%
     adjust-oml,%
     arrowhooks,%
     tie%
  }{mn-oml-#2}{}{}{}{}{}%
}

\installfonts
  \installopt{10}{Mixed}{}
  \installopt{7}{Mixed}{l1-}
  \installopt{10}{French}{}
  \installopt{7}{French}{l1-}
\endinstallfonts

\bye


==> fontinst/make-oml-medfamily-opticals.tex <==
\input fontinst-macros.tex

\def\installopt#1#2#3#4{%
  \installfont{MinionPro-#3#1-#4oml}{%
     MnSymbolA#2                       encoding mn-symbol-a,%
     MnSymbolC#2                       encoding mn-symbol-c,%
     MnSymbolD#2                       encoding mn-symbol-d,%
     MnSymbolE#2                       encoding mn-symbol-e,%
     MinionPro-#1-tosf-#4oml           encoding mn-oml-up,%
     MinionPro-It#1-tosf-#4oml         encoding mn-oml-it,%
     adjust-oml,%
     arrowhooks,%
     tie%
  }{mn-oml-#3}{}{}{}{}{}%
  \installfont{MinionPro-Semibold#3#1-#4oml}{%
     MnSymbolA-Bold#2                  encoding mn-symbol-a,%
     MnSymbolC-Bold#2                  encoding mn-symbol-c,%
     MnSymbolD-Bold#2                  encoding mn-symbol-d,%
     MnSymbolE-Bold#2                  encoding mn-symbol-e,%
     MinionPro-Semibold#1-tosf-#4oml   encoding mn-oml-up,%
     MinionPro-SemiboldIt#1-tosf-#4oml encoding mn-oml-it,%
     adjust-oml,%
     arrowhooks,%
     tie%
  }{mn-oml-#3}{}{}{}{}{}%
  \installfont{MinionPro-Bold#3#1-#4oml}{%
     MnSymbolA-Bold#2                  encoding mn-symbol-a,%
     MnSymbolC-Bold#2                  encoding mn-symbol-c,%
     MnSymbolD-Bold#2                  encoding mn-symbol-d,%
     MnSymbolE-Bold#2                  encoding mn-symbol-e,%
     MinionPro-Bold#1-tosf-#4oml       encoding mn-oml-up,%
     MinionPro-BoldIt#1-tosf-#4oml     encoding mn-oml-it,%
     adjust-oml,%
     arrowhooks,%
     tie%
  }{mn-oml-#3}{}{}{}{}{}%
}

\installfonts
  \installopt{Capt}{7}{Mixed}{l1-}
  \installopt{Capt}{7}{Mixed}{}
  \installopt{Subh}{12}{Mixed}{}
  \installopt{Disp}{12}{Mixed}{}
  \installopt{Capt}{7}{French}{l1-}
  \installopt{Capt}{7}{French}{}
  \installopt{Subh}{12}{French}{}
  \installopt{Disp}{12}{French}{}
\endinstallfonts

\bye


==> fontinst/make-oml-medfamily.tex <==
\input fontinst-macros.tex

\def\installopt#1#2#3{%
  \installfont{MinionPro-Semibold#2-#3oml}{%
     MnSymbolA-Bold#1                  encoding mn-symbol-a,%
     MnSymbolC-Bold#1                  encoding mn-symbol-c,%
     MnSymbolD-Bold#1                  encoding mn-symbol-d,%
     MnSymbolE-Bold#1                  encoding mn-symbol-e,%
     MinionPro-Semibold-tosf-#3oml     encoding mn-oml-up,%
     MinionPro-SemiboldIt-tosf-#3oml   encoding mn-oml-it,%
     adjust-oml,%
     arrowhooks,%
     tie%
  }{mn-oml-#2}{}{}{}{}{}%
}

\installfonts
  \installopt{10}{Mixed}{}
  \installopt{7}{Mixed}{l1-}
  \installopt{10}{French}{}
  \installopt{7}{French}{l1-}
\endinstallfonts

\bye


==> fontinst/make-oml-smallfamily.tex <==
\input fontinst-macros.tex

\def\installopt#1#2#3{%
  \installfont{MinionPro-#2-#3oml}{%
     MnSymbolA#1                       encoding mn-symbol-a,%
     MnSymbolC#1                       encoding mn-symbol-c,%
     MnSymbolD#1                       encoding mn-symbol-d,%
     MnSymbolE#1                       encoding mn-symbol-e,%
     MinionPro-Regular-tosf-#3oml      encoding mn-oml-up,%
     MinionPro-It-tosf-#3oml           encoding mn-oml-it,%
     adjust-oml,%
     arrowhooks,%
     tie%
  }{mn-oml-#2}{}{}{}{}{}%
  \installfont{MinionPro-Bold#2-#3oml}{%
     MnSymbolA-Bold#1                  encoding mn-symbol-a,%
     MnSymbolC-Bold#1                  encoding mn-symbol-c,%
     MnSymbolD-Bold#1                  encoding mn-symbol-d,%
     MnSymbolE-Bold#1                  encoding mn-symbol-e,%
     MinionPro-Bold-tosf-#3oml         encoding mn-oml-up,%
     MinionPro-BoldIt-tosf-#3oml       encoding mn-oml-it,%
     adjust-oml,%
     arrowhooks,%
     tie%
  }{mn-oml-#2}{}{}{}{}{}%
}

\installfonts
  \installopt{10}{Mixed}{}
  \installopt{7}{Mixed}{l1-}
  \installopt{10}{French}{}
  \installopt{7}{French}{l1-}
\endinstallfonts

\bye


==> mnsymbol/README <==
MnSymbol is a symbol font designed to be used in conjunction with Adobe
MinionPro.

All files in this archive are in the public domain.

WARNING
=======

This version includes a bugfix that causes incompatibilities with
previous versions. The symbols

  \...harpoonup and \...harpoondown

are now called

  \...harpoonccw and \...harpooncw

(This was needed for compatibility with amsfonts.sty.)

INSTALLATION
============

To install the fonts:

(0) If you have already a version of MnSymbol installed, delete the old
TFM and PK files.

(1) Run

  $ cd tex
  $ latex MnSymbol.ins

and copy the resulting file MnSymbol.sty to

   .../texmf/tex/latex/MnSymbol/MnSymbol.sty

(2) Copy all files in the "source" directory into the directory

   .../texmf/fonts/source/public/MnSymbol/

(3) Copy the documentation (MnSymbol.ps, MnSymbol.pdf, README) into the
directory

   .../texmf/doc/latex/MnSymbol/

(4) To install the PostScript fonts (courtesy of Michael Zedler) copy

  o enc/MnSymbol.map into .../texmf/fonts/map/dvips/MnSymbol
  o enc/*.enc        into .../texmf/fonts/enc/dvips/MnSymbol
  o pfb/*.pfb        into .../texmf/fonts/type1/public/MnSymbol

(These fonts are not strictly necessary but recommended.)

(5) You can copy the files in the "tfm" directory to

   .../texmf/fonts/tfm/public/MnSymbol

This is optional since these files can be generated automatically.
But it saves some time.

(6) Regenerate the file database:

  $ mktexlsr

If you installed the PostScript fonts you also need to run updmap or
updmap-sys to make them available:

  $ updmap-sys --enable MixedMap MnSymbol.map

(7) Happy TeXing.

Achim Blumensath


==> scripts/filltfm <==
#!/usr/bin/perl
# Fill the gaps in a given TFM with artifical characters.

use strict;
use warnings;

use File::Temp;

if (@ARGV != 2) {
    print STDERR "Usage: filltfm INPUT.tfm OUTPUT.tfm\n";
    exit(1);
}
my ($input, $output) = @ARGV;

open(PL, '-|', 'tftopl', '-charcode-format=octal', $input) or die $!;
my $tmp = new File::Temp(SUFFIX => '.pl');

my @char = ();
while (defined ($_ = <PL>)) {
    print $tmp $_;
    $char[oct($1)] = 1 if /CHARACTER O (\d+)/;
}
close(PL) or die $!;

for (grep !$char[$_], 0..255) {
    printf $tmp "(CHARACTER O %o)\n", $_;
}

close($tmp);
system('pltotf', $tmp, $output) and die $!;


==> scripts/filtererr <==
#!/usr/bin/perl
# Summarize maketfm's errors/warnings
#
# [r] I had to round some heights/depths (pltotf, vptovf); maxima at end
# [b] warning: no boundary character (otftotfm)
# [e] has no encoding, ignoring sth; summary of characters at end
use strict;
use warnings;
use List::Util qw(max);

my $show_round_flags = 0; # [r] appears almost everywhere
my $show_ignore_summary = 0; # whether to show what was ignored

my %errors = ();

sub flush_errors {
    print "]" if keys %errors;
    %errors = ();
}
sub print_literal {
    my $literal = shift;
    flush_errors() if length $literal;
    print $literal;
}
sub print_error {
    my $e = shift;
    print "[" unless keys %errors;
    if (!exists $errors{$e}) {
        print $e;
        $errors{$e}++;
    }
}

$| = 1;

my %rounded = (
    heights => 0,
    depths => 0,
    "italic corrections" => 0,
);
my %no_encoding = ();

while (<STDIN>) {
    s{(.*?)I had to round some (\w+(?:\s+\w+){0,2}) by ([\d.]+) units\.\n}[
        $rounded{$2} = max $rounded{$2}, $3;
        print_literal($1);
        print_error("r") if $show_round_flags;
        "";
    ]e;
    s{(.*?)otftotfm: warning: no boundary character.*?\n}[
        print_literal($1);
        print_error("b");
        "";
    ]e;
    s{(.*?)otftotfm: \(You may want to try.*?\)\n}[
        print_literal($1);
        print_error("b");
        "";
    ]e;
    s{(.*?)otftotfm:
        \ (
            \./enc/[\w-]+\.enckern # in a file
            |--ligkern\ command    # on the command line
        )
        (?::\d+)? # ignore line number
        :\ warning:\ '([\w.]+)'\ has\ no\ encoding,\ ignoring\ (.*)\n
    }[
        my ($where, $glyph, $ignoring) = ($2, $3, $4);
        print_literal($1);
        $no_encoding{$where}{$glyph}{$ignoring}++;
        print_error("e");
        "";
    ]xe;
    print_literal($_);
}
flush_errors();

foreach (sort keys %rounded) {
    if ($rounded{$_} > 0) {
	printf "I had to round some $_ by %.7f units.\n", $rounded{$_};
    }
}
foreach my $where (sort keys %no_encoding) {
    print "$where: warning: The following glyphs had no encoding: ";
    my @items;
    foreach my $glyph (sort keys %{$no_encoding{$where}}) {
        my $ignores = $no_encoding{$where}{$glyph};
        my $i = "$glyph";
        if ($show_ignore_summary) {
            $i .= " (ignoring " . (join ", ", sort keys %$ignores) . ")";
        }
        push @items, $i;
    }
    print join ", ", @items;
    print ".\n";
}


==> scripts/fix-map <==
#!/bin/bash
# Fix map lines referring to .otf fonts (resulting from otftotfm not finding
# the .pfb because they have not yet been installed: Happens either before the
# first installation if otftotfm is compiled with kpathsea support or in any
# case if it's compiled without.)
fix_map() {
    sed -e 's/\.otf$/.pfb/'
}

fix_map


==> scripts/makeall <==
#!/bin/bash

case "$*" in
  *--verbose*) verbose=true;;
  *)           verbose=false;;
esac

mkdir -p pfb tfm vf dvips

echo "Creating PostScript fonts ..."

for font in otf/*.otf
do
  base=$(basename "$font" .otf)
  cfftot1    "$font"     "$base.pfb"
  t1dotlessj "$base.pfb" "${base}LCDFJ.pfb"
done

echo "Creating TeX metrics ..."

maketfm() {
  local family="$1"
  shift

  # We pass the error code of maketfm via a stamp file.
  touch maketfm.error

  ( scripts/maketfm "$family" "$@" >"dvips/$family.map.tmp" && rm maketfm.error ) 2>&1 |
  ( ( ! $verbose && perl scripts/filtererr ) || cat )

  sed -e "s/\.otf$/.pfb/" <"dvips/$family.map.tmp" | sort -u >"dvips/$family.map"
  rm "dvips/$family.map.tmp"
}

maketfm MinionPro "$@"

mv *.pfb pfb

if [ -e maketfm.error ]
then
  rm maketfm.error
  echo "maketfm failed, exiting ..."
  exit 1
fi

(cd fontinst; ../scripts/makeint MinionPro; ../scripts/makeoml MinionPro)

(cd tex; latex MinionPro.ins; latex otfontdef.ins; latex fontaxes.ins)



==> scripts/maketfm <==
#!/bin/bash

# Check utilities.

otftotfm_version() {
  otftotfm --version | head -n 1 #| sed -e 's/^otftotfm .* \([0-9.]\+\)$/\1/'
}

requires_otftotfm_version() {

  local min_version="$1"
  local version="$(otftotfm_version)"

  version=${version#otftotfm (LCDF typetools) }

  : ${version:=0.0}

  local ver_major=${version%%.*}
  local ver_minor=${version#*.}
  local min_major=${min_version%%.*}
  local min_minor=${min_version#*.}

  if (( $ver_major < $min_major || ($ver_major == $min_major && $ver_minor < $min_minor) ))
  then
    echo "You need otftotfm version $min_version or greater to run this script." >&2
    exit 1
  fi
}

requires_otftotfm_version 2.62

# Parse options.

font="$1"

shift

usage() {
  exec >&2
  echo "USAGE: maketfm <font> [options]"
  echo -e "\nSupported options are:"
  echo "--verbose      | --quiet"
  echo "--smallcaps    | --nosmallcaps"
  echo "--swash        | --noswash"
  echo "--greek        | --nogreek"
  echo "--cyrillic     | --nocyrillic"
  echo "--vietnamese   | --novietnamese"
  echo "--kern         | --nokern"
  echo "--wide-spacing | --narrow-spacing"
  echo "--expanded     | --noexpanded"
  echo "--pack=<glyph list>"
  exit 1
}

if [[ "$font" == "" || "$font" == -* ]]
then
  echo -e "No font specified!\n" >&2
  usage
fi

verbose=false
create_greek=true
create_cyrillic=true
create_vietnamese=true
create_expanded=false
create_kerned=true
create_smallcaps=true
create_sc_grekcyrl=false
create_swash=true
wide_spacing=false
glyph_list=""
base_font_list=""

if ! otfinfo -f otf/$font-Regular.otf | grep -q smcp
then 
  create_smallcaps=false
fi

if ! otfinfo -f otf/$font-It.otf | grep -q Swash
then 
  create_swash=false
fi

for opt in "$@"
do
  case "$opt" in
    --verbose)        verbose=true;;
    --quiet)          verbose=false;;
    --greek)          create_greek=true;;
    --nogreek)        create_greek=false;;
    --smallcaps)      create_smallcaps=true;;
    --nosmallcaps)    create_smallcaps=false;;
    --swash)          create_swash=true;;
    --noswash)        create_swash=false;;
    --cyrillic)       create_cyrillic=true;;
    --nocyrillic)     create_cyrillic=false;;
    --vietnamese)     create_vietnamese=true;;
    --novietnamese)   create_vietnamese=false;;
    --expanded)       create_expanded=true;;
    --noexpanded)     create_expanded=false;;
    --kern)           create_kerned=true;;
    --nokern)         create_kerned=false;;
    --wide-spacing)   wide_spacing=true;;
    --narrow-spacing) wide_spacing=false;;
    --pack=*)         glyph_list="${opt#--pack=}";;
    --pack)           echo -e "Option --pack is missing an argument\n" >&2
                      usage;;
    *)                echo -e "Unknown option $opt\n" >&2
                      usage;;
  esac
done

# Expanded metrics for pdftex's font expansion.

if $create_expanded
then
  expansions="-20 -16 -12 -8 -4 0 4 8 12 16 20"
else
  expansions=0
fi

noliga="--unicoding='ff =: emptyslot'"
noliga="$noliga --unicoding='fi =: emptyslot'"
noliga="$noliga --unicoding='fl =: emptyslot'"
noliga="$noliga --unicoding='ffi =: emptyslot'"
noliga="$noliga --unicoding='ffl =: emptyslot'"

extra_flags=""
oml_flags=""
greek_flags=""
quote_flags=""
ts_it_compat_flags=""
ts_rm_compat_flags=""

make_lgr_flags() {
  for g in Iota iota upsilon lambda beta zeta eta Eta Gamma omicron alpha alphasub omegasub etasub epsilon psi gamma Mu Psi
  do
    echo -n " --unicoding 'space_dotbelowcomb_$g =: $1'"
  done
}

lgr_it_flags=$(make_lgr_flags uniE261)
lgr_rm_flags=$(make_lgr_flags uniE188)

if [ -e "scripts/maketfm-$font.cfg" ]
then
  . "scripts/maketfm-$font.cfg"
fi

# Output progress message later while the scripts run.

progress() {
  echo "echo $(printf "%q " "$@") >&2" >>maketfm.tmp
}

make_base_encodings() {

  if [[ $glyph_list != "" ]]
  then
    local i k n enc

    split -l 256 "$glyph_list" glyph-list.tmp-

    base_font_list=$(echo glyph-list.tmp-[a-z][a-z] | sed -e "s/glyph-list.tmp-//g")

    for i in $base_font_list
    do
      enc="dvips/base-$font-$i.enc"

      echo "% CODINGSCHEME FONTSPECIFIC" >"$enc"
      echo "/$font-Base-Encoding-$i [" >>"$enc"

      cat glyph-list.tmp-$i >>"$enc"

      n=$(wc -l <glyph-list.tmp-$i)

      for ((k = ${n// /}; k < 256; k++))
      do
        echo "/.notdef" >>"$enc"
      done

      echo "] def" >>"$enc"

      scripts/beautify-enc.sh "$enc"

      rm glyph-list.tmp-$i
    done
  fi
}

make_enckern() {

  if [ -e "$font-$1.pfb" ]
  then
    local e

    for e in enc/mn-*.enc
    do
      local enc=$(basename $e .enc)
      enc=${enc#mn-}

      for l in "" "-l1" "-l2"
      do
        if $create_kerned
        then
          if [ -e "kerning/$1$l-$enc.kern" ]
          then
            cat $e "kerning/$1$l-$enc.kern" | grep -v "#" >enc/mn-$1$l-$enc.enckern
          elif [ -e "kerning/$1$l.kern" ]
          then
            cat $e "kerning/$1$l.kern" | grep -v "#" >enc/mn-$1$l-$enc.enckern
          elif [ -e "kerning/$1-$enc.kern" ]
          then
            cat $e "kerning/$1-$enc.kern" | grep -v "#" >enc/mn-$1$l-$enc.enckern
          elif [ -e "kerning/$1.kern" ]
          then
            cat $e "kerning/$1.kern" | grep -v "#" >enc/mn-$1$l-$enc.enckern
          else
            cp $e enc/mn-$1$l-$enc.enckern
          fi
        else
          cp $e enc/mn-$1$l-$enc.enckern
        fi
      done
    done
  fi
}

get_exp_info() {
  local exp="$1"

  if (( exp == 0 ))
  then
    exp_suffix=""
    exp_factor=""
    exp_flags=""
  else
    exp_suffix=$(printf "%+d" "$exp")
    exp_factor=$(bc <<< "scale=3; 1+$exp/1000")
    exp_flags="-E $exp_factor"
  fi
}

make_base_fonts() {

  if [[ $glyph_list != "" ]]
  then
    local name="$1"
    local enc font_list i exp exp_flags exp_suffix exp_factor
    local common_flags="--tfm-directory=tfm --vf-directory=vf --encoding-directory=dvips --no-type1 --no-updmap"

    for exp in $expansions
    do
      get_exp_info "$exp"

      font_list="base-fonts-$font-$name$exp_suffix"

      echo -n "" >"$font_list"

      for i in $base_font_list
      do
        enc="dvips/base-$font-$i.enc"

        echo "$font-$name-Base-$i$exp_suffix $enc" >>"$font_list"

        otftotfm $common_flags $exp_flags --no-dotlessj --literal-encoding="$enc" "otf/$font-$name.otf" "$font-$name-Base-$i$exp_suffix"
      done

      # We also need to create a base font for the /dotlessj glyph.

      echo "$font-$name--lcdfj$exp_suffix - dotlessj" >>"$font_list"

      echo "$font-$name--lcdfj$exp_suffix $font-${name}LCDFJ \"${exp_factor:+$exp_factor ExtendFont}\" <$font-${name}LCDFJ.pfb"

      otftotfm $common_flags $exp_flags --no-map --encoding=enc/dotlessj.enc "otf/$font-$name.otf" "$font-$name$exp_suffix"

      rm "tfm/$font-$name$exp_suffix.tfm"
      rm "vf/$font-$name$exp_suffix.vf"
    done
  fi
}

get_base_encoding_flags () {
  if [[ "$base_font_list" != "" && "$2" != integral ]]
  then
    base_encoding_flags="--base-encodings='base-fonts-$font-$1$3'"
  else
    base_encoding_flags=""
  fi
}

get_enc_flags() {
  if [ "$2" != integral ]
  then
    case $3 in
      *-l2-*) enc_flags="-e 'enc/mn-$1-l2-$2.enckern'";;
      *-l1-*) enc_flags="-e 'enc/mn-$1-l1-$2.enckern'";;
      *)      enc_flags="-e 'enc/mn-$1-$2.enckern'";;
    esac
  else
    enc_flags="--literal-encoding enc/mn-integral.enc"
  fi
}

make_tfm() {

  local name="$1"
  local enc="$2"
  local spec="$3"
  shift 3

  local exp enc_flags base_encoding_flags exp_suffix exp_flags exp_factor

  get_enc_flags "$name" "$enc" "$spec"

  local common_flags="--tfm-directory=tfm --vf-directory=vf --encoding-directory=dvips"
  common_flags="$common_flags --no-type1 --no-updmap --no-dotlessj --warn-missing -fkern"
  if ! $verbose
  then
    common_flags="-q $common_flags"
  fi

  for exp in $expansions
  do
    get_exp_info "$exp"

    get_base_encoding_flags "$name" "$enc" "$exp_suffix"

    local tex_name="$font-$name-$spec$exp_suffix"

    if $verbose
    then
      progress -n " $tex_name,"
    else
      progress -n " $spec$exp_suffix,"
    fi

    echo "otftotfm $common_flags $base_encoding_flags $exp_flags $* $enc_flags 'otf/$font-$name.otf' '$tex_name'" >>maketfm.tmp
  done
}

make_ligkern_options() {
  if [ -e "kerning/$1.kern" ]
  then
    echo $(
      sed -n -e "s/#$2#//gp" "kerning/$1.kern" |
      awk '{print "--ligkern '\''"$3" "$4" "$5"'\''"}'
    )
  fi
}

get_flags() {
  case $2 in
      lf) flags="-flnum -fpnum";;
     osf) flags="-fonum -fpnum";;
     tlf) flags="-flnum -ftnum";;
    tosf) flags="-fonum -ftnum";;
  esac
  flags="$flags $quote_flags $(make_ligkern_options "$1" "$2")"
}
get_ts_flags() {
  case $1 in
    *It*) ts_flags="$ts_it_compat_flags";;
       *) ts_flags="$ts_rm_compat_flags";;
  esac
  case $2 in
      lf) ts_flags="$ts_flags -fpnum --subs-filter='<Number>' -fonum --subs-filter='!<Number>' -flnum";;
     osf) ts_flags="$ts_flags -fpnum --subs-filter='<Number>' -flnum --subs-filter='!<Number>' -fonum";;
     tlf) ts_flags="$ts_flags -ftnum --subs-filter='<Number>' -fonum --subs-filter='!<Number>' -flnum";;
    tosf) ts_flags="$ts_flags -ftnum --subs-filter='<Number>' -flnum --subs-filter='!<Number>' -fonum";;
  esac
}
get_sc_flags() {
  case $1 in
      lf) sc_flags="$noliga -flnum -fpnum --subs-filter='<Letter>' -fsmcp";;
     osf) sc_flags="$noliga -fonum -fpnum -fsmcp";;
     tlf) sc_flags="$noliga -flnum -ftnum --subs-filter='<Letter>' -fsmcp";;
    tosf) sc_flags="$noliga -fonum -ftnum -fsmcp";;
  esac
}
get_sc_ts_flags() {
  case $1 in
    *It*) sc_ts_flags="$ts_it_compat_flags";;
       *) sc_ts_flags="$ts_rm_compat_flags";;
  esac
  case $2 in
      lf) sc_ts_flags="$sc_ts_flags -fpnum"
          sc_ts_flags="$sc_ts_flags --subs-filter='<Number>'  -fonum"
          sc_ts_flags="$sc_ts_flags --subs-filter='!<Number>' -flnum"
          sc_ts_flags="$sc_ts_flags --subs-filter='<Letter>'  -fsmcp";;
     osf) sc_ts_flags="$sc_ts_flags -fpnum -fsmcp"
          sc_ts_flags="$sc_ts_flags --subs-filter='<Number>'  -flnum"
          sc_ts_flags="$sc_ts_flags --subs-filter=!'<Number>' -fonum";;
     tlf) sc_ts_flags="$sc_ts_flags -ftnum"
          sc_ts_flags="$sc_ts_flags --subs-filter='<Number>'  -fonum"
          sc_ts_flags="$sc_ts_flags --subs-filter='!<Number>' -flnum"
          sc_ts_flags="$sc_ts_flags --subs-filter='<Letter>'  -fsmcp";;
    tosf) sc_ts_flags="$sc_ts_flags -ftnum -fsmcp"
          sc_ts_flags="$sc_ts_flags --subs-filter='<Number>'  -flnum"
          sc_ts_flags="$sc_ts_flags --subs-filter='!<Number>' -fonum";;
  esac
}
get_it_ot1_flags() {
  case "$1" in
    *It*) it_ot1_flags="--unicoding 'dollar =: sterling'";;
    *)    it_ot1_flags="";;
  esac
}
get_lgr_flags() {
  case "$1" in
    *It*) lgr_flags="--unicoding 'kappa =: kappasymbolgreek kappa' --unicoding 'theta =: theta1 theta' $lgr_it_flags $greek_flags";;
    *)    lgr_flags="$lgr_rm_flags $greek_flags";;
  esac
}

make_normal_metrics() {

  get_flags        "$1" "$2"
  get_ts_flags     "$1" "$2"
  get_sc_flags     "$2"
  get_sc_ts_flags  "$1" "$2"
  get_it_ot1_flags "$1"
  get_lgr_flags    "$1"

  make_tfm   "$1" t1  $2-t1  "-fliga $flags"
  make_tfm   "$1" ot1 $2-ot1 "-fliga $it_ot1_flags $flags"
  make_tfm   "$1" ly1 $2-ly1 "-fliga $flags"
  make_tfm   "$1" ts1 $2-ts1 "       $ts_flags"

  if $create_greek
  then
    make_tfm "$1" lgr $2-lgr "-sgrek $lgr_flags $flags"
    make_tfm "$1" lgi $2-lgi "-sgrek $lgr_flags $flags"
  fi
  if $create_cyrillic
  then
    make_tfm "$1" t2a $2-t2a "-scyrl $flags"
    make_tfm "$1" t2b $2-t2b "-scyrl $flags"
    make_tfm "$1" t2c $2-t2c "-scyrl $flags"
    make_tfm "$1" x2  $2-x2  "-scyrl $flags"
    make_tfm "$1" ot2 $2-ot2 "-scyrl $flags"
  fi
  if $create_vietnamese
  then
    make_tfm "$1" t5   $2-t5 "       $flags"
  fi

  if $create_smallcaps
  then
    make_tfm     "$1" t1   $2-sc-t1     "       $sc_flags               --unicoding='germandbls =: SSsmall'"
    make_tfm     "$1" ot1  $2-sc-ot1    "       $sc_flags $it_ot1_flags --unicoding='germandbls =: SSsmall' --unicoding='dotlessj =: Jsmall'"
    make_tfm     "$1" ly1  $2-sc-ly1    "       $sc_flags               --unicoding='germandbls =: SSsmall' --unicoding='dotlessj =: Jsmall'"
    make_tfm     "$1" ts1  $2-sc-ts1    "       $sc_ts_flags"

    make_tfm     "$1" t1   $2-sc-l2-t1  "-L 80  $sc_flags               --space-factor=1.15 --unicoding='germandbls =: SSsmall'"
    make_tfm     "$1" ot1  $2-sc-l2-ot1 "-L 80  $sc_flags $it_ot1_flags --space-factor=1.15 --unicoding='germandbls =: SSsmall' --unicoding='dotlessj =: Jsmall'"
    make_tfm     "$1" ly1  $2-sc-l2-ly1 "-L 80  $sc_flags               --space-factor=1.15 --unicoding='germandbls =: SSsmall' --unicoding='dotlessj =: Jsmall'"
    make_tfm     "$1" ts1  $2-sc-l2-ts1 "-L 80  $sc_ts_flags            --space-factor=1.15"

    if $create_sc_grekcyrl
    then
      if $create_greek
      then
        make_tfm "$1" lgr  $2-sc-lgr    "       $sc_flags               -sgrek $lgr_flags"
        make_tfm "$1" lgi  $2-sc-lgi    "       $sc_flags               -sgrek $lgr_flags"
        make_tfm "$1" lgr  $2-sc-l2-lgr "-L 80  $sc_flags               -sgrek $lgr_flags --space-factor=1.15 "
        make_tfm "$1" lgi  $2-sc-l2-lgi "-L 80  $sc_flags               -sgrek $lgr_flags --space-factor=1.15"
      fi
      if $create_cyrillic
      then
        make_tfm "$1" t2a  $2-sc-t2a    "       $sc_flags               -scyrl"
        make_tfm "$1" t2b  $2-sc-t2b    "       $sc_flags               -scyrl"
        make_tfm "$1" t2c  $2-sc-t2c    "       $sc_flags               -scyrl"
        make_tfm "$1" x2   $2-sc-x2     "       $sc_flags               -scyrl"
        make_tfm "$1" ot2  $2-sc-ot2    "       $sc_flags               -scyrl"
        make_tfm "$1" t2a  $2-sc-l2-t2a "-L 80  $sc_flags               -scyrl --space-factor=1.15"
        make_tfm "$1" t2b  $2-sc-l2-t2b "-L 80  $sc_flags               -scyrl --space-factor=1.15"
        make_tfm "$1" t2c  $2-sc-l2-t2c "-L 80  $sc_flags               -scyrl --space-factor=1.15"
        make_tfm "$1" x2   $2-sc-l2-x2  "-L 80  $sc_flags               -scyrl --space-factor=1.15"
        make_tfm "$1" ot2  $2-sc-l2-ot2 "-L 80  $sc_flags               -scyrl --space-factor=1.15"
      fi
    fi

    if $create_vietnamese
    then
      make_tfm   "$1" t5   $2-sc-t5     "       $sc_flags"
      make_tfm   "$1" t5   $2-sc-l2-t5  "-L 80  $sc_flags               --space-factor=1.15"
    fi
  fi
}

make_spread_metrics() {

  get_flags        "$1" "$2"
  get_ts_flags     "$1" "$2"
  get_sc_flags     "$2"
  get_sc_ts_flags  "$1" "$2"
  get_it_ot1_flags "$1"
  get_lgr_flags    "$1"

  make_tfm "$1" t1     $2-l1-t1     "-L 40        $flags"
  make_tfm "$1" ot1    $2-l1-ot1    "-L 40        $it_ot1_flags $flags"
  make_tfm "$1" ly1    $2-l1-ly1    "-L 40        $flags"
  make_tfm "$1" ts1    $2-l1-ts1    "-L 40        $ts_flags"

  if $create_greek
  then
    make_tfm "$1" lgr  $2-l1-lgr    "-L 40 -sgrek $lgr_flags $flags"
    make_tfm "$1" lgi  $2-l1-lgi    "-L 40 -sgrek $lgr_flags $flags"
  fi
  if $create_cyrillic
  then
    make_tfm "$1" t2a  $2-l1-t2a    "-L 40 -scyrl $flags"
    make_tfm "$1" t2b  $2-l1-t2b    "-L 40 -scyrl $flags"
    make_tfm "$1" t2c  $2-l1-t2c    "-L 40 -scyrl $flags"
    make_tfm "$1" x2   $2-l1-x2     "-L 40 -scyrl $flags"
    make_tfm "$1" ot2  $2-l1-ot2    "-L 40 -scyrl $flags"
  fi
  if $create_vietnamese
  then
    make_tfm "$1" t5   $2-l1-t5     "-L 40        $flags"
  fi

  if $create_smallcaps
  then
    make_tfm     "$1" t1  $2-sc-l1-t1  "-L 40 $sc_flags               --unicoding='germandbls =: SSsmall'"
    make_tfm     "$1" ot1 $2-sc-l1-ot1 "-L 40 $sc_flags $it_ot1_flags --unicoding='germandbls =: SSsmall' --unicoding='dotlessj =: Jsmall'"
    make_tfm     "$1" ly1 $2-sc-l1-ly1 "-L 40 $sc_flags               --unicoding='germandbls =: SSsmall' --unicoding='dotlessj =: Jsmall'"
    make_tfm     "$1" ts1 $2-sc-l1-ts1 "-L 40 $sc_ts_flags"

    if $create_sc_grekcyrl
    then
      if $create_greek
      then
        make_tfm "$1" lgr  $2-sc-l1-lgr "-L 40 $sc_flags -sgrek $lgr_flags"
        make_tfm "$1" lgi  $2-sc-l1-lgi "-L 40 $sc_flags -sgrek $lgr_flags"
      fi
      if $create_cyrillic
      then
        make_tfm "$1" t2a  $2-sc-l1-t2a "-L 40 $sc_flags -scyrl"
        make_tfm "$1" t2b  $2-sc-l1-t2b "-L 40 $sc_flags -scyrl"
        make_tfm "$1" t2c  $2-sc-l1-t2c "-L 40 $sc_flags -scyrl"
        make_tfm "$1" x2   $2-sc-l1-x2  "-L 40 $sc_flags -scyrl"
        make_tfm "$1" ot2  $2-sc-l1-ot2 "-L 40 $sc_flags -scyrl"
      fi
    fi

    if $create_vietnamese
    then
      make_tfm   "$1" t5   $2-sc-l1-t5  "-L 40 $sc_flags"
    fi
  fi
}

make_integrals() {

  if [ -e "$font-$1.pfb" ]
  then
    progress -n "Processing font $font-$1 ..."

    cp enc/mn-integral.enc dvips

    make_tfm "$1" integral integral
    make_tfm "$1" integral integral-cn1 "-E 0.85"
    make_tfm "$1" integral integral-cn2 "-E 0.75 -S 0.04"

    progress " done."
  fi
}

make_metrics() {

  if [ -e "$font-$1.pfb" ]
  then
    progress -n "Processing font $font-$1 ..."

    make_base_fonts "$1"

    make_normal_metrics "$1" lf
    make_normal_metrics "$1" tlf
    make_normal_metrics "$1" osf
    make_normal_metrics "$1" tosf

    make_tfm "$1" oml     tosf-oml "-L 40 --math-spacing=255 --subs-filter='!uniF638' -fonum -ftnum $oml_flags"
    make_tfm "$1" extra-u extra-u  "$extra_flags"

    progress " done."
  fi
}

make_spaced_metrics() {

  if [ -e "$font-$1.pfb" ]
  then
    progress -n "Processing font $font-$1 ..."

    make_spread_metrics "$1" lf
    make_spread_metrics "$1" tlf
    make_spread_metrics "$1" osf
    make_spread_metrics "$1" tosf

    make_tfm "$1" oml tosf-l1-oml "-L 80 --math-spacing=255 --subs-filter='!uniF638' -fonum -ftnum $oml_flags"

    progress " done."
  fi
}

make_swash_metrics() {

  if [ -e "$font-$1.pfb" ]
  then
    progress -n "Processing font $font-$1 ..."

    get_it_ot1_flags "$1"

    local swash="--include-alternates '*.swash' -faalt"

    make_tfm   "$1" t1  lf-swash-t1    "-fliga -flnum -fpnum $swash"
    make_tfm   "$1" t1  osf-swash-t1   "-fliga -fonum -fpnum $swash"
    make_tfm   "$1" t1  tlf-swash-t1   "-fliga -flnum -ftnum $swash"
    make_tfm   "$1" t1  tosf-swash-t1  "-fliga -fonum -ftnum $swash"
    make_tfm   "$1" ot1 lf-swash-ot1   "-fliga -flnum -fpnum $it_ot1_flags $swash"
    make_tfm   "$1" ot1 osf-swash-ot1  "-fliga -fonum -fpnum $it_ot1_flags $swash"
    make_tfm   "$1" ot1 tlf-swash-ot1  "-fliga -flnum -ftnum $it_ot1_flags $swash"
    make_tfm   "$1" ot1 tosf-swash-ot1 "-fliga -fonum -ftnum $it_ot1_flags $swash"
    make_tfm   "$1" ly1 lf-swash-ly1   "-fliga -flnum -fpnum $swash"
    make_tfm   "$1" ly1 osf-swash-ly1  "-fliga -fonum -fpnum $swash"
    make_tfm   "$1" ly1 tlf-swash-ly1  "-fliga -flnum -ftnum $swash"
    make_tfm   "$1" ly1 tosf-swash-ly1 "-fliga -fonum -ftnum $swash"

    if $create_vietnamese
    then
      make_tfm "$1" t5  lf-swash-t5    "-flnum -fpnum $swash"
      make_tfm "$1" t5  osf-swash-t5   "-fonum -fpnum $swash"
      make_tfm "$1" t5  tlf-swash-t5   "-flnum -ftnum $swash"
      make_tfm "$1" t5  tosf-swash-t5  "-fonum -ftnum $swash"
    fi

    progress " done."
  fi
}

make_spaced_swash_metrics() {

  if [ -e "$font-$1.pfb" ]
  then
    progress -n "Processing font $font-$1 ..."

    get_it_ot1_flags "$1"

    local swash="--include-alternates '*.swash' -faalt"

    make_tfm   "$1" t1  lf-swash-l1-t1    "-L 40 -flnum -fpnum $swash"
    make_tfm   "$1" t1  osf-swash-l1-t1   "-L 40 -fonum -fpnum $swash"
    make_tfm   "$1" t1  tlf-swash-l1-t1   "-L 40 -flnum -ftnum $swash"
    make_tfm   "$1" t1  tosf-swash-l1-t1  "-L 40 -fonum -ftnum $swash"
    make_tfm   "$1" ot1 lf-swash-l1-ot1   "-L 40 -flnum -fpnum $it_ot1_flags $swash"
    make_tfm   "$1" ot1 osf-swash-l1-ot1  "-L 40 -fonum -fpnum $it_ot1_flags $swash"
    make_tfm   "$1" ot1 tlf-swash-l1-ot1  "-L 40 -flnum -ftnum $it_ot1_flags $swash"
    make_tfm   "$1" ot1 tosf-swash-l1-ot1 "-L 40 -fonum -ftnum $it_ot1_flags $swash"
    make_tfm   "$1" ly1 lf-swash-l1-ly1   "-L 40 -flnum -fpnum $swash"
    make_tfm   "$1" ly1 osf-swash-l1-ly1  "-L 40 -fonum -fpnum $swash"
    make_tfm   "$1" ly1 tlf-swash-l1-ly1  "-L 40 -flnum -ftnum $swash"
    make_tfm   "$1" ly1 tosf-swash-l1-ly1 "-L 40 -fonum -ftnum $swash"

    if $create_vietnamese
    then
      make_tfm "$1" t5  lf-swash-l1-t5    "-L 40 -flnum -fpnum $swash"
      make_tfm "$1" t5  osf-swash-l1-t5   "-L 40 -fonum -fpnum $swash"
      make_tfm "$1" t5  tlf-swash-l1-t5   "-L 40 -flnum -ftnum $swash"
      make_tfm "$1" t5  tosf-swash-l1-t5  "-L 40 -fonum -ftnum $swash"
    fi

    progress " done."
  fi
}

make_series() {

  local sub

  for sub in "" Capt Disp Subh
  do
    if [[ "$1$sub" = "" ]]
    then
      make_enckern Regular
      make_metrics Regular
    else
      make_enckern "$1$sub"
      make_metrics "$1$sub"
    fi
  done

  make_spaced_metrics "$1Capt"

  if [[ "$1" = "" ]]
  then
    make_spaced_metrics Regular
  else
    make_spaced_metrics "$1"
  fi
}

make_additional_italic() {

  local sub

  for sub in "" Capt Disp Subh
  do
    if $create_swash
    then
      make_swash_metrics "$1$sub"
    fi
    make_integrals       "$1$sub"
  done

  if $create_swash
  then
    make_spaced_swash_metrics "$1"
    make_spaced_swash_metrics "$1Capt"
  fi
}

# Ok, let's start.

make_base_encodings

# We first create a shell script with the actual otftotfm calls.

echo "#!/bin/bash" >maketfm.tmp

for weight in Light "" Medium Semibold Bold Black
do
  for width in Cond SemiCn "" SemiExt
  do
    make_series             "$weight$width"
    make_series             "$weight${width}It"

    make_additional_italic  "$weight${width}It"
  done
done

# Then we execute and delete it.

tr "\177" " " <maketfm.tmp >maketfm.tmp2  # This is just a workaround for a bug on some systems.

. maketfm.tmp2

rm -f maketfm.tmp maketfm.tmp2 base-fonts-"$font"-*


